Efficient Search for Customized Activation Functions with Gradient Descent

Different activation functions work best for different deep learning models. To exploit this, we leverage recent advancements in gradient-based search techniques for neural architectures to efficiently identify high-performing activation functions for a given application. We propose a fine-grained search cell that combines basic mathematical operations to model activation functions, allowing for the exploration of novel activations. Our approach enables the identification of specialized activations, leading to improved performance in every model we tried, from image classification to language models. Moreover, the identified activations exhibit strong transferability to larger models of the same type, as well as new datasets. Importantly, our automated process for creating customized activation functions is orders of magnitude more efficient than previous approaches. It can easily be applied on top of arbitrary deep learning pipelines and thus offers a promising practical avenue for enhancing deep learning architectures.

==> sections/pseudocodes.tex <==

\begin{algorithm}[h]
\begin{algorithmic}
\STATE \textbf{Input:} \\
    \STATE\hspace{\algorithmicindent} - One-shot model with initialized network weights $w$ and architecture parameters $\alpha$
    \STATE\hspace{\algorithmicindent} - Train and validation loss functions $\mathcal{L}_{train}$ and $\mathcal{L}_{valid}$
   \STATE\hspace{\algorithmicindent} - $e_{max}$, $t_{max}$
    \STATE{\textbf{Set:} $e=0, t=0$}
\WHILE{$e < e_{max}$ \& architecture not discretized} 
\STATE{Perform one step of DrNAS algorithm}
 \STATE{\textbf{if:} argmax($\alpha_{0}$) $=$ argmax($\alpha_t$) \textbf{then:} \\
 \hspace{4mm} $t \mathrel{+}= 1$ \\
 \textbf{else:} \\
 \hspace{4mm} $t = 0$} \\
 \textbf{end if}
 \STATE{\textbf{if:} $t$ > $t_{max}$ \textbf{then:} \\
  \hspace{4mm} remove the worst half of operations based on $\alpha$ values \\
  \hspace{4mm} $t = 0$} \\
 \textbf{end if}
\ENDWHILE
\RETURN Activation function based on fully discretized operations 
\STATE Train model with selected activation from scratch
\end{algorithmic}
\caption{DrNAS with gradual pruning} % - Differentiable Architecture Search
\label{alg:optim1}
\end{algorithm}  

\begin{algorithm}[h]
\begin{algorithmic}
\STATE \textbf{Input:} \\
    \STATE\hspace{\algorithmicindent} - One-shot model with initialized network weights $w$ and architecture parameters $\theta$
    \STATE\hspace{\algorithmicindent} - Train and validation loss functions $\mathcal{L}_{train}$ and $\mathcal{L}_{valid}$
    \STATE\hspace{\algorithmicindent} - $e_{max}$, $t_{max}$
    \STATE{\textbf{Set:} $e=0, t=0$}
\WHILE{$e < e_{max}$ \& architecture not discretized} 
\STATE{$\alpha_t$ (activation parameters) = output of MLP($\theta$)}
\STATE{Perform one step of DARTS algorithm, optimizing MLP weights $\theta$ in the outer loop}
 \STATE{\textbf{if:} argmax($\alpha_{0}$) $=$ argmax($\alpha_t$) \textbf{then:} \\
 \hspace{4mm} $t \mathrel{+}= 1$ \\
 \textbf{else:} \\
 \hspace{4mm} $t = 0$} \\
 \textbf{end if}
 \STATE{\textbf{if:} $t$ > $t_{max}$ \textbf{then:} \\
  \hspace{4mm} remove the worst half of operations based on $\alpha$ values \\
  \hspace{4mm} $t = 0$} \\
 \textbf{end if}
\ENDWHILE
\RETURN Activation function based on fully discretized operations 
\STATE Train model with selected activation from scratch
\end{algorithmic}
\caption{DARTS with gradual pruning} % - Differentiable Architecture Search
\label{alg:optim2}
\end{algorithm}  


\begin{algorithm}[h]
\begin{algorithmic}
\STATE \textbf{Input:} \\
    \STATE\hspace{\algorithmicindent} - One-shot model with initialized network weights $w$ and architecture parameters $\alpha$
    \STATE\hspace{\algorithmicindent} - Train and validation loss functions $\mathcal{L}_{train}$ and $\mathcal{L}_{valid}$
\WHILE{\textit{not converged}} 
\STATE{
	1. Update architecture $\alpha$ by descending  $\nabla_\alpha \mathcal{L}_{valid}(w - \xi \nabla_w \mathcal{L}_{train}(w, \alpha), \alpha)$ \\ 
	 \phantom{2.} ($\xi =0$ if using first-order approximation) \\
	2. Update weights $w$ by descending $\nabla_w \mathcal{L}_{train}(w, \alpha)$} 
\ENDWHILE

\STATE Derive the final architecture based on argmax of learned $\alpha$
\STATE Train the architecture from scratch
\end{algorithmic}
\caption{DARTS - Differentiable Architecture Search}
\label{alg:darts}
\end{algorithm}  




\begin{algorithm}[h]
	\begin{algorithmic}
        \STATE \textbf{Input:} \\
    \STATE\hspace{\algorithmicindent} - One-shot model with Initialized weights $w$ \\
    \STATE\hspace{\algorithmicindent} - Dirichlet distribution parameters $\beta$. \\
    \STATE\hspace{\algorithmicindent} - Anchor $\hat \beta=1$, anchor regularizer parameter $\lambda$, and metric $d$
		\WHILE{\textit{not converged}} 
		\STATE{
			1. Update distribution parameters $\beta$ by descending  $\nabla_\beta\big(E_{\theta \sim Dir(\beta)}[\mathcal{L}_{valid}(w, \theta)]+ \lambda d(\beta, \hat \beta)\big)$ \\
			2. Sample architecture paremeters $\theta \sim Dir(\beta)$ \\ 
			3. Update weights $w$ by descending $\nabla_w \mathcal{L}_{train}(w, \theta)$} 
		\ENDWHILE
		\STATE Derive the final architecture based on argmax of learned $\beta$
		\STATE Train the architecture from scratch
	\end{algorithmic}
	\caption{DrNAS - Dirichlet Neural Architecture Search}
	\label{alg: drnas}
\end{algorithm}


